TedNet: A Pytorch Toolkit for Tensor Decomposition Networks

Tensor Decomposition Networks (TDNs) prevail for their inherent compact architectures. To give more researchers a flexible way to exploit TDNs, we present a Pytorch toolkit named TedNet. TedNet implements 5 kinds of tensor decomposition(i.e., CANDECOMP/PARAFAC (CP), Block-Term Tucker (BTT), Tucker-2, Tensor Train (TT) and Tensor Ring (TR) on traditional deep neural layers, the convolutional layer and the fully-connected layer. By utilizing the basic layers, it is simple to construct a variety of TDNs. TedNet is available at https://github.com/tnbar/tednet.

==> content/usage.tex <==
\section{Installation and Usage}

There are two ways to install TedNet. For the sake that the source code of TedNet is submitted to GitHub, it is feasible to install from the downloaded code by command \textbf{python setup.py install}. Compared with aforementioned fussy way, another one, the recommended way is to install TedNet trough PyPI~\footnote{https://pypi.org/project/tednet} by command \textbf{pip install tednet}. After installation, all tensor decomposition models of TedNet can be used.

An example of Tensor Ring is shown in Listing~\ref{ll:tr}. Tensor ring decomposition can be used by import module \textbf{tednet.tnn.tensor\_ring}. The usage of other decomposition is the same and more details can be found in the Document~\footnote{https://tednet.readthedocs.io}.

% \begin{figure}[h]
% \centering
% \subfloat[Tensor Ring Models]{
%     % \caption{Interest region}
%     \includegraphics[width=0.48\columnwidth]{figures/tr-usage.png}
%     \label{fig:tr-usage}
% }
% \subfloat[Tensor Train Models]{
%     % \caption{Performance}
%     \includegraphics[width=0.48\columnwidth]{figures/tt-usage.png}
%     \label{fig:tt-usage}
% }
% \caption{Usage of TedNet.}
% \label{fig:usage}
% \end{figure}

% \lstinputlisting[
%     % style       =   Python,
%     caption     =   {\bf Tensor Ring Models},
%     label       =   {cd:tr}
% ]{codes/tr.py}

\begin{lstlisting}[language={Python}, label={ll:tr}, caption={\bf The Usage of Tensor Ring Models}]
# import tensor ring module
import tednet.tnn.tensor_ring as tr

# TR-LSRM
model = tr.TRLSTM([16, 16], [32, 32], [5, 5, 5, 5])

# TR-Lenet-5
model = tr.TRLeNet5(10, [6, 6, 6, 6])

# TR-ResNet-20
model = tr.TRResNet20([7, 7, 7, 7, 7, 7, 7], 10)
\end{lstlisting}


